Aspectuality Across Genre: A Distributional Semantics Approach

The interpretation of the lexical aspect of verbs in English plays a crucial role for recognizing textual entailment and learning discourse-level inferences. We show that two elementary dimensions of aspectual class, states vs. events, and telic vs. atelic events, can be modelled effectively with distributional semantics. We find that a verb's local context is most indicative of its aspectual class, and demonstrate that closed class words tend to be stronger discriminating contexts than content words. Our approach outperforms previous work on three datasets. Lastly, we contribute a dataset of human--human conversations annotated with lexical aspect and present experiments that show the correlation of telicity with genre and discourse goals.

==> asp_ambig_analysis_pos.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l}
\textbf{Context} & \textbf{PoS group} \\ \hline
win-1 & \texttt{IN}: $71.7 \, (490/683)$, \texttt{*DT}: $70.9 \, (368/519)$, \\
		& \texttt{PRP*}: $76.4 \, (246/322)$, \texttt{NN*}: $73.7 \, (207/281)$, \\ 
		& \texttt{*RB*}: $74.5 \, (137/184)$ \\ \hline

dep (full) 	& \texttt{NN*}: $67.3 \, (638/948)$, \texttt{VB*}: $71.5 \, (243/340)$, \\
		&  \texttt{JJ*}: $67.0 \, (65/97)$, \texttt{*RB*}: $82.2 \, (60/73)$, \\
		&  \texttt{PRP*}: $78.8 \, (52/66)$\\
\end{tabular}}
\captionsetup{font=small}
\caption{ANALYSIS ON THE ASP AMBIG DATASET.}
\label{tbl:asp_ambig_analysis_pos}
\end{table}

==> asp_ambig_analysis_words.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l}
\textbf{Context} & \textbf{Words} \\ \hline
win-1 & \emph{the}: $72.2 \, (197/273)$, \emph{in}: $68.5 \, (89/130)$, \\
		& \emph{with}: $67.4 \, (62/92)$, \emph{that}: $79.8 \, (71/89)$, \\ 
		& \emph{it}: $70.4 \, (50/71)$ \\ \hline

dep (full) 	& \emph{it}: $78.3 \, (18/23)$, \emph{god}: $50.0 \, (5/10)$, \\
		& \emph{her}: $88.9 \, (8/9)$, \emph{be}: $55.6 \, (5/9)$, \\
		&  \emph{needs}: $50.0 \, (4/8)$ \\
\end{tabular}}
\captionsetup{font=small}
\caption{ANALYSIS ON THE ASP AMBIG DATASET.}
\label{tbl:asp_ambig_analysis_words}
\end{table}

==> asp_ambig_results.tex <==
\begin{table}[!htb]
%\setlength{\belowcaptionskip}{-5pt}
%\setlength{\abovecaptionskip}{-2pt}
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | c c}
\textbf{Model} & \textbf{Accuracy} \\ \hline
verb-only & $65.9$  \\\hline
% infer-sent
window-1 & $\textbf{74.2}$ \\
window-3 & $72.4$ \\
window-5 & $71.4$ \\ \hline
dependency (head only) & $66.1$  \\
dependency (children only) & $70.3$ \\
dependency (full) & $70.1$  \\\hline
full sentence & $69.6$ \\\hline
%full sentence (tf-idf) & $69.1$ & $39.4$  \\\hline\hline % TODO: Change to standard majority class stats
majority class & $65.9$ \\
\texttt{CAEVO} TimeML & $55.6$ \\
% caevo (all) & $17.6$ & $11.2$ \\
% caevo (predicted only) & $59.6$ & $32.1$ \\
\cite{Friedrich_2014} & $72.0$ \\
\cite{Heuschkel_2016} & $72.8$ \\%\hline
\end{tabular}%}
\captionsetup{font=small}
\caption{Results on \textbf{Asp-ambig} \emph{state} vs. \emph{event}.}
\label{tbl:asp_ambig_results}
\end{table}

==> asp_ambig_results_per_verb.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | c | c | c | c | c}
\textbf{Verb} & \textbf{Majority class} & \textbf{\citet{Friedrich_2014}} & \textbf{\citet{Heuschkel_2016}} & \textbf{window-1} & \textbf{dependency (full)}\\ \hline
\emph{feel} 		& $\textbf{96.1}$ & $93.8$ & $95.5$ & $94.2$ & $93.5$ \\
\emph{say} 		& $\textbf{94.9}$ & $93.5$ & $94.2$ & $\textbf{94.9}$ & $\textbf{94.9}$\\
\emph{make} 		& $91.9$ & $91.2$ & \textbf{$92.0$} & $90.6$ & $90.6$ \\
\emph{come} 		& $\textbf{88.0}$ & $87.2$ & $\textbf{88.0}$ & $85.5$ & $86.2$\\
\emph{take} 		& $85.4$ & $85.4$ & $85.5$ & $85.5$ & $\textbf{87.0}$\\
\emph{meet} 		& $83.9$ & $87.7$ & $85.9$ & $87.7$ & $\textbf{90.6}$\\
\emph{stand} 		& $80.0$ & $83.1$ & $81.8$ & $\textbf{87.7}$ & $82.6$\\
\emph{find} 		& $74.5$ & $68.8$ & $\textbf{76.6}$ & $75.4$ & $69.6$\\
\emph{accept} 		& $\textbf{70.9}$ & $65.7$ & $67.4$ & $68.8$ & $61.6$\\
\emph{hold} 		& $56.0$ & $49.3$ & $57.8$ & $\textbf{62.3}$ & $55.8$ \\
\emph{carry} 		& $55.9$ & $58.1$ & $60.3$ & $58.0$ & $\textbf{63.8}$\\
\emph{look} 		& $55.8$ & $74.6$ & $65.9$ & $\textbf{79.7}$ & $61.6$\\
\emph{show} 		& $54.9$ & $\textbf{68.4}$ & $65.9$ & $67.4$ & $65.2$\\
\emph{appear} 		& $52.2$ & $61.0$ & $56.6$ & $\textbf{70.3}$ & $62.3$\\
\emph{follow} 		& $51.6$ & $65.6$ & $61.8$ & $61.6$ & $\textbf{69.6}$ \\
\emph{consider} 	& $50.7$ & $70.3$ & $67.4$ & $\textbf{77.5}$ & $59.4$\\
\emph{cover} 		& $50.4$ & $54.5$ & $55.0$ & $\textbf{57.2}$ & $50.0$\\
\emph{fill} 			& $47.8$ & $62.7$ & $\textbf{69.4}$ & $60.1$ & $48.6$\\
\emph{bear} 		& $47.4$ & $67.4$ & $\textbf{77.2}$ & $68.1$ & $63.8$\\
\emph{allow} 		& $37.8$ & $\textbf{51.9}$ & $51.1$ & $50.7$ & $44.9$\\\hline
Average			& $66.3$ & $72.0$ & $72.8$ & $\textbf{74.2}$ & $70.1$ \\
\end{tabular}}
\captionsetup{font=small}
\caption{Per verb Accuracies on the \textbf{Asp-ambig} dataset~\citep{Friedrich_2014}.}
\label{tbl:asp_ambig_results_per_verb}
\end{table}

==> asp_ambig_results_with_f1.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 (macro)} \\ \hline
verb-only & $65.9$ & $27.6$  \\\hline
% infer-sent
window-1 & $\textbf{74.2}$ & $48.4$ \\
window-3 & $72.4$ & $\textbf{48.7}$ \\
window-5 & $71.4$ & $48.3$ \\ \hline
dependency (head only) & $66.1$ & $35.8$  \\
dependency (children only) & $70.3$ & $44.8$ \\
dependency (full) & $70.1$ & $45.5$  \\\hline
full sentence & $69.6$ & $41.9$ \\\hline\hline
%full sentence (tf-idf) & $69.1$ & $39.4$  \\\hline\hline % TODO: Change to standard majority class stats
majority class & $65.9$ & $27.6$ \\
\texttt{CAEVO} & $55.6$ & $33.0$ \\
% caevo (all) & $17.6$ & $11.2$ \\
% caevo (predicted only) & $59.6$ & $32.1$ \\
\citet{Friedrich_2014} & $72.0$ & $-$ \\
\citet{Heuschkel_2016} & $72.8$ & $-$ \\%\hline
\end{tabular}}
\captionsetup{font=small}
\caption{Results on the \textbf{Asp-ambig} dataset~\citep{Friedrich_2014}.}
\label{tbl:asp_ambig_results}
\end{table}

==> aspect-exp.tex <==
In our first set of experiments, we aim to build models for predicational aspect classification solely on the basis of distributional word representations, and investigate what contexts are most predictive for determining predicational aspect. Figure~\ref{fig:model_overview} shows the overall XXX of our approach. In the following we describe the kinds of context we consider, the composition functions and the classifier, and the datasets on which we evaluate our models. Detailed parameterisations for each model are presented in Appendix YYY.

\begin{figure*}[!htb]
%\setlength{\belowcaptionskip}{-5pt}
%\setlength{\abovecaptionskip}{-2pt}
\includegraphics[width=\textwidth]{./_resources/model_overview.png}
\captionsetup{font=small}
\caption{For a given input sentence we extract the target verb's context and compose it into a fixed size vector representation. This representation is subsequently used as input to a classifier that determines the predicational aspect of input phrase.}
\label{fig:model_overview}
\end{figure*}

\subsection{Context}

We analyse the kinds of contexts that are most indicative of the predicational aspect of a verb phrase. In this paper we consider two different kinds of context: a linear window-based context, e.g. one word to the left and one word to the right of the target verb, and a dependency-based context window which leverages the syntactic structure of the verb phrase. Considering the input sentence with the target verb \emph{decided} in Figure~\ref{fig:example_sentence_context}, for example, would result in extracted context words \emph{Jane} and \emph{to} for a linear context window, and in \emph{Jane} and \emph{leave} for a dependency-based context window.

\begin{figure}[!htb]
\setlength{\belowcaptionskip}{-5pt}
\setlength{\abovecaptionskip}{-2pt}
\centering
\begin{dependency}
\begin{deptext}[column sep=0.7cm]
  \small{Jane}\&
    \small{\emph{decided}}\& 
      \small{to}\&
        \small{leave}\&
          \small{early}\\
\end{deptext}
\deproot{2}{root}
\depedge{2}{1}{nsubj}
\depedge{2}{4}{xcomp}
\depedge{4}{3}{aux}
\depedge{4}{5}{advmod}
\end{dependency}
\captionsetup{font=small}
\caption{With a linear context window of size $1$, \emph{Jane} and \emph{to} would be extracted as contexts for the verb \emph{decided}. With a dependency-based context, \emph{Jane} and \emph{leave} would be extracted.}
\label{fig:example_sentence_context}
\end{figure}
We furthermore use the target verb without any context and the full sentence as baseline comparisons.

\subsection{Composition Functions}

We consider three ways of composing a target verb with its context and describe each one in turn below. All composition functions receive GloVe~\citep{Pennington_2014} embeddings as input.

\textbf{Vector average.} Composing word vectors by adding or averaging has been shown to be a very strong baseline for a variety of problems~\citep{Iyyer_2015,Wieting_2016b,Kober_2017}. Recent work~\citep{Tian_2017} has shown that the sum or average of two neural word embeddings approximates the intersection of the corresponding feature spaces. Averaging word vectors is a task-independent composition function and we assess whether a simple function is sufficient for reliably determining predicational aspect.

\textbf{LSTM encoder.} We furthermore consider a bidirectional LSTM~\citep{Hochreiter_1997} encoder (biLSTM) as composition function. A biLSTM encoder represents a more powerful composition function, which is trained jointly with the subsequent classifier in an end-to-end fashion, thereby representing a task-specific composition function.

\textbf{BERT.} Lastly we consider BERT~\citep{Devlin_2019}, which has been shown to achieve impressive performance on numerous NLP tasks. BERT is a sentence encoder model based on the Transformer~\citep{Vaswani_2017} architecture that uses multi-headed bidirectional self-attention and a novel training objective in order to overcome the sequential limitation of RNN based encoders. We use BERT as a composition function in order to assess its ability to encode predicational aspect in its representations.

All composition functions return a fixed size vector representation of the target verb, composed with its context, which we subsequently pass into a classifier.

\subsection{Classifier and Baselines}

As classifier we consider a feedforward network that receives the composed representation of a verb phrase as input and predicts the predicational aspect of the phrase. Appendix ZZZ shows the parameterisation of the feedforward network for each dataset. We use two baseline models for comparison: a logistic regression classifier\footnote{We use scikit-learn~\citep{Pedregosa_2011} and use \texttt{liblinear} as solver and otherwise the default hyperparameter settings.} that receives averaged word embeddings as input (henceforth ``\textbf{LR-Base}") and a feedforward network that receives the embedding of the verb without any context (henceforth ``\textbf{FF-Verb}"). Following~\citep{Friedrich_2014} we furthermore report the results of a majority class baseline.

\subsection{Datasets}

We evaluate our methods on 3 datasets, which focus on the distinction between a verb in context expressing a \emph{state} vs. an \emph{event}. We use the \textbf{Asp-ambig} dataset introduced by~\citet{Friedrich_2014}. The dataset contains 20 frequently occurring verbs whose predicational aspect commonly changes depending on context. For each verb,~\citet{Friedrich_2014} collected 138 sentences from the Brown Corpus~\citep{Francis_1979}. In total the dataset contains 2760 instances, where each target verb is labelled as  expressing a \emph{state}, an \emph{event}, or \emph{both}\footnote{The instances labelled as \emph{both} have either been labelled by the annotators as \emph{both} because both readings are possible, or have been labelled as \emph{both} when the annotators disagreed in their judgement~\citep{Friedrich_2014}.}. Following~\citet{Friedrich_2014}, we report Accuracy\footnote{A performance overview per verb type is included Appendix~\ref{sec:supplemental_a}.} using \emph{leave-one-out} cross-validation.

We furthermore evaluate our approach on the \emph{Situation Entities} (\textbf{SitEnt}) dataset~\citep{Friedrich_2016}. The \textbf{SitEnt} dataset contains $\approx$40k sentences from the MASC corpus~\citep{Ide_2008} and English Wikipedia, split into separate training and test sets. We evaluate our approach on the test set, using the original split of~\citet{Friedrich_2016}. The \textbf{SitEnt} dataset is a 2-class problem with target verbs being either labelled as \emph{state} or \emph{event}, but not as \emph{both} as in the \textbf{Asp-ambig} dataset. We report Accuracy as well as a per-class F1-score.

In the \textbf{SitEnt} dataset we noticed that only around 20\% of the verb types in the training set occur with both labels, and only around 5\% have a balanced\footnote{The class distribution has a bias of at most 60:40 towards the majority class.} (i.e. ambiguous) label distribution. This characteristic of the dataset could lead to the problem of any classifier overfitting on the correlation between specific verbs and their unambiguous labels, rather than learning the types of contexts necessary for determining predicational aspect. We therefore downsampled the original dataset, keeping only verb types that occur with both labels, and randomly subsampled the majority class for verb types with an imbalanced class distribution. The new dataset, ``\textbf{SitEnt-ambig}", consists of 6547 examples in the training set and 1402 examples in the test set\footnote{All our resources are available from \url{website}}. We evaluate performance on the \textbf{SitEnt-ambig} test set in two different ways, by firstly training the models on the whole \textbf{SitEnt} training set, and secondly by training the models on the smaller \textbf{SitEnt-ambig} training set. We report Accuracy and the per-class F1-scores.

\subsection{Results}

Table~\ref{tbl:aspect_results_by_model} shows the results of our best performing models in comparison to previous results across all datasets. Our models achieve a new state-of-the-art on the \textbf{Asp-ambig} and \textbf{SitEnt} datasets and outperform the other models on the subsampled \textbf{SitEnt-ambig} dataset. 

Notably, the performance of our \textbf{LR-Base} and \textbf{FF-Verb} baselines is very strong on the \textbf{Asp-ambig} and \textbf{SitEnt} datasets and is competitive with previous results from the literature. Looking at the results of the \textbf{FF-Verb} baseline on the \textbf{SitEnt} dataset confirms our suspicion that the often unambiguous verb-label distribution has a significant effect on model performance as the results on the \textbf{SitEnt-ambig} dataset show. 

Across the board, model performance drops by around 20 points when moving from \textbf{SitEnt} to \textbf{SitEnt-ambig}, with BERT being slightly more robust than the other models. In all cases, learning a model on the \textbf{SitEnt-ambig} dataset produced stronger results than training on the larger \textbf{SitEnt} dataset, providing further evidence of the models exploiting the unambiguous verb-label distribution artefact.
\input{./_tables/aspect_results_by_model.tex}

In general, \textbf{SitEnt-ambig} reflects a very pessimistic and --- arguably unrealistically --- hard scenario, and therefore a lower bound on performance of classifying predicational aspect with models based on distributional semantics. Our results indicate that the models perform well when confronted with a more natural scenario as in the \textbf{SitEnt} dataset, however they fail to leverage enough contextual information to reliably classify predicational aspect in a more difficult setting, leaving much leeway for improvements for future work.

\subsection{Analysis}

\subsubsection{Window vs. Dependency Context}

We first contrast performance between the best model using a linear context window and the best model utilising the dependency context around a target verb\footnote{We omit BERT from this comparison because it is unclear how it can operate over a syntactic tree.}. Figure~\ref{fig:window_vs_dependency} shows that with only one exception, a the words within a linear context window around the target verb are stronger indicators of predicational aspect.  

\begin{figure}[!htb]
\setlength{\belowcaptionskip}{-3pt}
\setlength{\abovecaptionskip}{-2pt}
\includegraphics[width=\columnwidth]{./_resources/window_vs_dependency.png}
\captionsetup{font=small}
\caption{WINDOW VS DEPENDENCY.}
\label{fig:window_vs_dependency}
\end{figure}

As Figure~\ref{fig:extracted_context_by_pos} shows, linear context windows predominantly consist of closed class words such as determiners, prepositions or pronouns, whereas dependency based contexts primarily extract verbs or nouns.

\begin{figure}[!htb]
\setlength{\belowcaptionskip}{-3pt}
\setlength{\abovecaptionskip}{-2pt}
\includegraphics[width=\columnwidth]{./_resources/win_vs_dep_pos_tags.png}
\captionsetup{font=small}
\caption{EXTRACTED POS TAGS.}
\label{fig:extracted_context_by_pos}
\end{figure}

The superior performance of window-based contexts over dependency-based ones, and the PoS distribution of extracted contexts suggests that closed class words are a better indicator of predicational aspect than content words. We therefore calculate the accuracy per PoS tag, which is the proportion of a context with a particular PoS tag being part of a correct classification decision, and we subsequently average these scores for closed class PoS tags and open class PoS tags\footnote{See Appendix XXX for a list of which PoS tags count as closed class and which as open class.}. Figure~\ref{fig:avg_acc_per_pos} indeed shows that closed class contexts typically are more reliable than content words for determining predicational aspect. This result furthermore shows that the often complex semantics of closed class words can --- to some extent --- be captured by distributional representations and leveraged for determining predicational aspect. For example, sentences~\ref{ex:look_event}-\ref{ex:stand_state} below from the \textbf{SitEnt} and \textbf{Asp-ambig} datasets show how the presence of verb particles is indicative of an event (sentences~\ref{ex:look_event}-\ref{ex:stand_state}), whereas their absence (sentences~\ref{ex:look_state}-\ref{ex:stand_state}) suggests a state.

\begin{enumerate}[label={(\arabic*)}, series=qa]
\itemsep0em
\item \label{ex:look_event} Shane \emph{looked at} his watch. (\textbf{event})
\item \label{ex:stand_event} Jefferson shook his head and \emph{stood up}. (\textbf{event})
\item \label{ex:look_state} She sure \emph{looks} good. (\textbf{state})
\item \label{ex:stand_state} A metal table and four chairs \emph{stood} in the center. (\textbf{state})
\end{enumerate}

The significance of particles for determining predicational aspect might not be too surprising as in languages such as German, the particles are part of the verb itself, and even in English they are closely coupled with the word almost to the extent that \emph{look at} or \emph{stand up} can effectively be considered a single word. However, the fact that distributional representations of words such as \emph{at} or \emph{up} possess the discriminatory power for determining predicational aspect is a very interesting finding of our experiments. While particles tend to be highly indicative of events, we have found pleonastic pronouns in a subject position and existential \emph{there}'s to be strong predictors of stative predicational aspect\footnote{See Appendix ABC for Accuracy scores on a per-word basis.}.  

\begin{figure}[!htb]
\setlength{\belowcaptionskip}{-3pt}
\setlength{\abovecaptionskip}{-2pt}
\includegraphics[width=\columnwidth]{./_resources/avg_acc_per_pos.png}
\captionsetup{font=small}
\caption{EXTRACTED POS TAGS.}
\label{fig:avg_acc_per_pos}
\end{figure}

\subsubsection{Context Window Size}

AT MOST 3 WORDS, MORE BAD

FOR THE LINEAR CONTEXT WINDWO WE INVESTIGATE WHAT SIZE OF WINDOW PRODUCES THE BEST RESULTS

\begin{figure*}[!htb]
\setlength{\belowcaptionskip}{-3pt}
\setlength{\abovecaptionskip}{-2pt}
\centering
\includegraphics[width=0.8\textwidth]{./_resources/accuracy_by_context_window_size.png}
\captionsetup{font=small}
\caption{EXTRACTED POS TAGS.}
\label{fig:accuracy_by_context_window_size}
\end{figure*}

LOCAL CLAUSE LEVEL, RATHER THAN ANYTHING LARGER

EXISTENTIAL THERE / PLEONASTIC PRONOUN, VERY INDICATIVE OF STATIVE CONTEXTS


SAY THAT PREDICATIONAL ASPECT SHOULD BE MODELLED ON THE CLAUSE LEVEL RATHER THAN THE SENTENCE LEVEL AS IT DEPENDS ON ITS LOCAL CONTEXT, GLOBAL CONTEXT NOT SO IMPORTANT

==> aspect-methods.tex <==
%The utility of distributional semantic word representations --- both high-dimensional count-based, and low-dimensional neural word embeddings --- has been shown in a large body of works in recent years at the lexical~\citep{Baroni_2014,Weeds_2014b,Roller_2016,Nguyen_2017}, as well as the sentence level~\citep{Socher_2013b,Bowman_2015,Mihaylov_2017}. In order to contextualise a verb within a phrase we apply pointwise addition as a simple distributional composition function. Pointwise addition in neural word embeddings approximates the intersection of their contexts~\citep{Tian_2017}, and has been shown to be an efficient function for contextualising a word with its phrasal context~\citep{Arora_2016,Kober_2017}. 
The utility of distributional semantic word representations has been shown in a large body of works  in recent years (\citet{Weeds_2014b,Nguyen_2017,Socher_2013b,Bowman_2015}; \emph{inter alia}). In order to compose a verb with its context we apply pointwise addition as a simple distributional composition function. Pointwise addition in neural word embeddings approximates the intersection of their contexts~\citep{Tian_2017}, and has been shown to be an efficient function for contextualising a word in a phrase~\citep{Arora_2016,Kober_2017}. 

\subsection{Classifiers and Embeddings}

Following previous work on modelling the aspectual class of a verb~\citep{Siegel_2000,Friedrich_2014}, we treat the problem as a supervised classification task, $y = f(x)$, where $y$ represents the aspectual class of a verb, $f$ represents a classifier, and $x$ an input vector representation. For all of our experiments, $f$ is a logistic regression classifier with default hyperparameter settings using \texttt{scikit-learn}~\citep{Pedregosa_2011}, and the input vector $x$ is based on $300$-dimensional pre-trained skip-gram \texttt{word2vec}~\citep{Mikolov_2013b} vectors\footnote{\url{https://code.google.com/archive/p/word2vec/}}. We lowercase all words, but do not apply any other form of morphological preprocessing.

\subsection{Verb-Only Aspect}

For this approach we obtain a \texttt{word2vec} representation $x$ for a given verb $v$ and feed $x$ into a logistic regression classifier in order to predict the aspectual class of $v$. The underlying assumption of this approach is that the aspectual class of a verb is a purely lexical phenomenon that can be captured by its distributional semantic representation, and does not require the integration of any context of the current phrase.

\subsection{Context-Rich Aspect}

Let $x$ be a \texttt{word2vec} representation for a given verb $v$, and $C$ be the set of context words extracted for $v$, with $c \in C$ denoting the vector representation for a context word. The composed representation of $v$, denoted by $x^{\prime}$, can then be expressed as a simple sum:
\begin{equation}
\label{eqn:composition}
	x^{\prime} = x + \sum_{c \in C}{c}
\end{equation}
Subsequently, $x^{\prime}$ is passed through a logistic regression classifier in order to predict the aspectual class of $v$. The rationale behind this model is that the local context of a given verb is able to determine the aspectual class of $v$.

\subsubsection{Types of Context}

We investigate two different types of context: simple linear context windows of varying length and first-order dependency contexts. For example for the sentence in Figure~\ref{fig:example_sentence_context}, a linear context window of size $1$ would extract \emph{Jane} and \emph{to} for the target verb \emph{decided}, whereas a dependency-based context would extract \emph{Jane} and \emph{leave}. We used the Stanford NLP pipeline~\citep{Manning_2014} with default settings for parsing. 

\begin{figure}[!htb]
\setlength{\belowcaptionskip}{-5pt}
\setlength{\abovecaptionskip}{-2pt}
\centering
\begin{dependency}
\begin{deptext}[column sep=0.7cm]
  \small{Jane}\&
    \small{\emph{decided}}\& 
      \small{to}\&
        \small{leave}\&
          \small{early}\\
\end{deptext}
\deproot{2}{root}
\depedge{2}{1}{nsubj}
\depedge{2}{4}{xcomp}
\depedge{4}{3}{aux}
\depedge{4}{5}{advmod}
\end{dependency}
\captionsetup{font=small}
\caption{With a linear context window of size $1$, \emph{Jane} and \emph{to} would be extracted as contexts for the verb \emph{decided}. With a dependency-based context, \emph{Jane} and \emph{leave} would be extracted.}
\label{fig:example_sentence_context}
\end{figure} 
For linear context windows we use sizes \{1, 3, 5\}, and for first-order dependency-based contexts we experiment with using only the head\footnote{If the target verb is the root, then no context is used for that verb.} of the verb, only its children, or the full first-order context. 

\subsubsection{Incorporating the Full Sentence}

We furthermore test a model that incorporates the whole sentential context into a vector representation. The approach simply uses all words from a given sentence and composes their corresponding \texttt{word2vec} representations as in Equation~\ref{eqn:composition} to create a sentence embedding. Adding word vectors for deriving sentence representations has been shown to be an effective method for other NLP tasks such as Sentiment Analysis~\citep{Iyyer_2015} or Recognising Textual Entailment~\citep{Wieting_2016b}.

The underlying rationale behind this approach is that the aspectual class of a verb is a function of the sentence as a whole, rather than dependent on local context alone~\citep{Moens_1987,Dowty_1991}.%TIME PERMITTING INFERSENT ENCODER % https://github.com/facebookresearch/InferSent

==> closed_class_indicators.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ l | l}
\textbf{Dataset} & \textbf{Lexeme (Accuracy)} \\ \hline
Asp-ambig	& \emph{like} $(94.1)$, \emph{at} $(92.9)$, \emph{out} $(92.3)$\\%, \\
%			& \emph{up} $(88.0)$, \emph{them} $(85.7)$ \\\hline
SitEnt	& \emph{there} $(96.8)$, \emph{an} $(93.6)$, \emph{will} $(92.2)$\\ %, \\
%		& \emph{would} $(92.9)$, \emph{you} $(92.4)$ \\\hline
SitEnt-ambig	& \emph{can} $(93.8)$,  \emph{are} $(84.4)$, \emph{up} $(77.8)$\\ %, \\
%			& \emph{at} $(77.2)$, \emph{we} $(69.6)$ \\\hline
Telicity	& \emph{me} $(96.4)$, \emph{that} $(96.2)$, \emph{you} $(96.2)$\\ %, \\
%		& \emph{she} $(95.3)$, \emph{her} $(95.2)$ \\\hline
Telicity-ambig	& \emph{that} $(88.9)$, \emph{he} $(72.2)$, \emph{the} $(72.2)$\\ %, \\
%			& \emph{she} $(71.1)$, \emph{not} $(71.4)$ \\
\end{tabular}}
\captionsetup{font=small}
\caption{Top $3$ most indicative closed class words.}
\label{tbl:closed_class_indicators}
\end{table}

==> open_vs_closed_class.tex <==
\begin{table}[!htb]
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l | l}
\textbf{Dataset} & \textbf{Dependency} & \textbf{Window} \\ \hline
\textbf{Asp-ambig} 	& \emph{closed class}: $77.1$ & \emph{closed class}: $72.3$ \\
				& \emph{open class}: $69.0$ & \emph{open class}: $74.6$ \\\hline
\textbf{SitEnt}	& \emph{closed class}: $79.9$ & \emph{closed class}: $83.5$ \\
			& \emph{open class}: $77.8$ & \emph{open class}: $81.4$ \\\hline
\textbf{SitEnt-ambig}	& \emph{closed class}: $65.0$ & \emph{closed class}: $59.4$ \\
				& \emph{open class}: $61.7$ & \emph{open class}: $59.3$ \\\hline
\textbf{Telicity}	& \emph{closed class}: $82.1$ & \emph{closed class}: $86.5$ \\
			& \emph{open class}: $79.6$ & \emph{open class}: $83.0$ \\\hline
\textbf{Telicity-ambig}	& \emph{closed class}: $78.6$ & \emph{closed class}: $66.7$ \\
					& \emph{open class}: $77.5$ & \emph{open class}: $61.4$ \\
\end{tabular}%}
\captionsetup{font=small}
\caption{ANALYSIS OPEN VS CLOSED CLASS.}
\label{tbl:open_vs_closed_class}
\end{table}

==> sitent_analysis_ambiguous_pos.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l | l}
\textbf{Context} & \textbf{PoS group SitEnt} & \textbf{PoS group SitEnt-ambig} \\ \hline

win-1	& \texttt{NN*+VB*}: $80.1 \, (3193/3988)$, & \texttt{NN*+VB*}: $60.0 \, (478/797)$, \\
		&\texttt{PRP*+*DT}: $86.4 \, (3035/3514)$ & \texttt{IN+PRP*}: $58.9 \, (438/744)$ \\\hline

dep (full) 	& \texttt{NN*+VB*}: $77.7 \, (8968/11535)$, & \texttt{NN*+VB*}: $62.1 \, (1520/2448)$,\\ 
		& \texttt{PRP*+CC}: $80.3 \, (2219/2765)$  & \texttt{PRP*+CC}: $65.0 \, (396/609)$\\
\end{tabular}}
\captionsetup{font=small}
\caption{ANALYSIS ON THE SITENT DATASET.}
\label{tbl:sitent_analysis_ambiguous_pos}
\end{table}

==> sitent_analysis_pos.tex <==
\begin{table}[!htb]
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l}
\textbf{Context} & \textbf{PoS group} \\ \hline
win-1 & \texttt{NN*+VB*}: $80.1 \, (3193/3988)$, \\ &\texttt{PRP*+*DT}: $86.4 \, (3035/3514)$ \\\hline
dep (full) 	& \texttt{NN*+VB*}: $77.7 \, (8968/11535)$, \\ & \texttt{PRP*+CC}: $80.3 \, (2219/2765)$ \\
\end{tabular}%}
\captionsetup{font=small}
\caption{ANALYSIS ON THE SITENT DATASET.}
\label{tbl:sitent_analysis_pos}
\end{table}

==> sitent_results.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ l | c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 (state)} & \textbf{F1 (event)} \\ \hline
verb-only & $\textbf{85.4}$ & $\textbf{84.0}$ & $\textbf{86.6}$ \\\hline
% VERB ONLY LEMMA & $83.6$ & $81.8$ & $85.0$ \\
% infer-sent
window-1 & $82.8$ & $81.2$ & $84.1$\\
% WINDOW 1 LEMMA & $79.1$ & $77.9$ & $80.2$ \\
window-3 & $80.0$ & $78.2$ & $81.5$\\
window-5 & $76.6$ & $74.5$ & $78.4$\\ \hline
dependency (head only) & $83.1$ & $81.3$ & $84.5$ \\
dependency (children only) & $80.7$ & $79.1$ & $82.2$ \\
dependency (full) & $80.7$ & $79.1$ & $82.2$ \\\hline
% DEPENDENCY FULL LEMMA & $76.3$ & $76.5$ & $76.1$ \\
full sentence & $70.8$ & $67.4$ & $73.5$ \\\hline
%full sentence (tf-idf) & $69.9$ & $67.3$ & $72.1$ \\\hline
majority class & $52.6$ & $0.0$ & $68.9$ \\
\texttt{CAEVO} TimeML & $59.2$ & $32.2$ & $70.9$ \\
\cite{Friedrich_2016} & $-$ & $80.6$ & $78.6$ \\%\hline
\end{tabular}}
\captionsetup{font=small}
\caption{Results on \textbf{SitEnt} \emph{state} vs. \emph{event}.}
\label{tbl:sitent_results}
\end{table}

==> sitent_results_ambiguous.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ l | c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 (state)} & \textbf{F1 (event)} \\ \hline
verb-only & $55.0$ & $44.0$ & $62.4$ \\
window-1 & $59.1$ & $54.9$ & $62.5$\\
dependency (full) & $\textbf{61.3}$ & $\textbf{60.0}$ & $62.4$ \\\hline
majority class & $52.0$ & $0.0$ & $\textbf{68.4}$ \\
\texttt{CAEVO} TimeML & $53.9$ & $24.9$ & $66.8$ \\
% caevo 47.4 & 0.0 & 64.3
\end{tabular}}
\captionsetup{font=small}
\caption{Results on \textbf{SitEnt-ambig} \emph{state} vs. \emph{event}.}
\label{tbl:sitent_results_ambiguous}
\end{table}

==> sitent_results_lemma.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 (state)} & \textbf{F1 (event)} \\ \hline
verb only & $85.4$ & $84.0$ & $86.6$ \\
verb lemma & $83.6 (-1.8)$ & $81.8 (-2.2)$ & $85.0 (-1.6)$ \\\hline
win-1 & $82.8$ & $81.2$ & $84.1$\\
win-1 lemma & $79.1 (-3.7)$ & $77.9 (-3.2)$ & $80.2 (-3.9)$ \\\hline
dep (full) & $80.7$ & $79.1$ & $82.2$ \\
dep (full) lemma & $76.3 (-4.4)$ & $76.5 (-2.6)$ & $76.1 (-6.1)$ \\
\end{tabular}}
\captionsetup{font=small}
\caption{RESULTS ON THE SITENT DATASET~\citep{Friedrich_2016}.}
\label{tbl:sitent_results_lemma}
\end{table}

==> telicity_analysis_ambiguous_pos.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l | l}
\textbf{Context} & \textbf{PoS group Telicity} & \textbf{PoS group Telicity-ambig} \\ \hline

win-1	& \texttt{PRP*+IN}: $87.1 \, (1054/1210)$, & \texttt{PRP*+IN*}: $76.1 \, (150/197)$, \\
		&\texttt{NN*+VB*}: $82.5 \, (719/871)$ & \texttt{NN*+RB*}: $65.9 \, (89/135)$ \\\hline

dep (full) 	& \texttt{NN*+VB*}: $79.5 \, (3362/4231)$, & \texttt{NN*+VB*}: $65.4 \, (421/651)$,\\ 
		& \texttt{PRP*+CC}: $83.4 \, (1071/1284)$  & \texttt{PRP*+CC}: $70.9 \, (188/265)$\\
\end{tabular}}
\captionsetup{font=small}
\caption{ANALYSIS ON THE TELICITY DATASET.}
\label{tbl:telicity_analysis_ambiguous_pos}
\end{table}

==> telicity_results.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ l | c c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1} & \textbf{F1 (telic)} & \textbf{F1 (atelic)} \\ \hline
verb-only & $\textbf{87.4}$ & $\textbf{78.7}$ & $\textbf{92.2}$ & $\textbf{65.2}$ \\\hline
% VERB LEMMA & $86.4$ & $75.5$ & $91.7$ & $59.4$
% infer-sent
window-1 & $86.8$ & $76.5$ & $91.8$ & $61.1$\\
% WINDOW 1 LEMMA & $84.8$ & $73.1$ & $90.6$ & $55.5$
%window-2 & $82.7$ & $70.7$ & $89.1$ & $52.3$\\
window-3 & $81.8$ & $69.8$ & $88.5$ & $51.1$\\
window-5 & $80.4$ & $67.9$ & $87.4$ & $48.4$\\ \hline
dep (head only) & $85.3$ & $74.4$ & $90.8$ & $58.1$ \\
dep (children only) & $83.8$ & $72.3$ & $89.8$ & $54.8$ \\
dep (full) & $82.0$ & $69.2$ & $88.6$ & $49.8$ \\\hline
full sentence & $77.9$ & $63.3$ & $86.3$ & $40.3$ \\\hline
%full sentence (tf-idf) & $82.0$ & $45.0$ & $90.1$ & $0.0$ \\
majority class & $82.0$ & $45.0$ & $90.1$ & $0.0$ \\
FG2017 (basic) & $86.7$ & $74.5$ & $\textbf{92.2}$ & $53.7$ \\
FG2017 (+InterCorp) & $82.3$ & $76.4$ & $88.6$ & $61.4$\\
\end{tabular}}
\captionsetup{font=small}
\caption{Results on \textbf{Telicity}.}
\label{tbl:telicity_results}
\end{table}

==> telicity_results_ambiguous.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{ l | c c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1} & \textbf{F1 (telic)} & \textbf{F1 (atelic)} \\ \hline
verb-only & $63.4$ & $44.2$ & $76.9$ & $11.5$ \\
% VERB LEMMA & $86.4$ & $75.5$ & $91.7$ & $59.4$
% infer-sent
window-1 & $68.1$ & $54.1$ & $79.5$ & $28.8$\\
% WINDOW 1 LEMMA & $84.8$ & $73.1$ & $90.6$ & $55.5$
dependency (full) & $\textbf{72.9}$ & $\textbf{62.2}$ & $82.3$ & $\textbf{42.0}$ \\\hline
majority class & $72.5$ & $42.0$ & $\textbf{84.1}$ & $0.0$ \\
\end{tabular}}
\captionsetup{font=small}
\caption{Results on \textbf{Telicity-ambig}.}
\label{tbl:telicity_results_ambiguous}
\end{table}

==> telicity_results_lemma.tex <==
\begin{table}[!htb]
\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | c c c c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1} & \textbf{F1 (telic)} & \textbf{F1 (atelic)} \\ \hline
verb only & $\textbf{87.4}$ & $\textbf{78.7}$ & $\textbf{92.2}$ & $\textbf{65.2}$ \\
verb lemma & $86.4$ & $75.5$ & $91.7$ & $59.4$ \\\hline
win-1 & $86.8$ & $76.5$ & $91.8$ & $61.1$\\
win-1 lemma & $84.8$ & $73.1$ & $90.6$ & $55.5$ \\\hline
dep (full) & $82.0$ & $69.2$ & $88.6$ & $49.8$ \\
dep (full) lemma & $80.4$ & $66.5$ & $87.9$ & $45.2$\\
\end{tabular}}
\captionsetup{font=small}
\caption{RESULTS ON THE TELICITY DATASET~\citep{Friedrich_2017}.}
\label{tbl:results_telicity_lemma}
\end{table}

==> timebank_label_mapping.tex <==
\begin{table}[!htb]
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l}
\textbf{TimeBank Annotation} & \textbf{This Work} \\ \hline
\texttt{ASPECTUAL} & Event \\
\texttt{I\_ACTION} & Event \\
\texttt{I\_STATE} & State \\
\texttt{OCCURRENCE} & Event \\
\texttt{PERCEPTION} & State \\
\texttt{REPORTING} & Event \\
\texttt{STATE} & State \\
\end{tabular}%}
\captionsetup{font=small}
\caption{Aspectual class annotation mapping between TimeBank and this work.}
\label{tbl:timebank_label_mapping}
\end{table}

==> walking_around_example_1.tex <==
\begin{table*}[!htb]
%\setlength{\belowcaptionskip}{-5pt}
%\setlength{\abovecaptionskip}{-2pt}
\centering
\small
%\resizebox{\textwidth}{!}{
\begin{tabular}{ l l}
Speaker 1 & \emph{So (..) can you (..) the first place you have to go to is called the Cedar Plaque, do you know what that is?} \\
Speaker 2 & \emph{Nope} \\
Speaker 1 & \emph{Okay, so um (..) do you know where the Humanities is?} \\
Speaker 2 & \emph{Yes} \\
Speaker 1 & \emph{Okay, so walk out of the Psych building and towards the Humanities fountain.} \\
Speaker 2 & \emph{Okay} \\
...
\end{tabular}%}
\caption{Part of an example dialogue from the Walking Around corpus~\cite{Brennan_2013}.}
\label{tbl:walking_around_example}
\end{table*}
